Hyperspectral Unmixing in Presence of Endmember Variability, Nonlinearity or Mismodelling Effects

This paper presents three hyperspectral mixture models jointly with Bayesian algorithms for supervised hyperspectral unmixing. Based on the residual component analysis model, the proposed general formulation assumes the linear model to be corrupted by an additive term whose expression can be adapted to account for nonlinearities (NL), endmember variability (EV), or mismodelling effects (ME). The NL effect is introduced by considering a polynomial expression that is related to bilinear models. The proposed new formulation of EV accounts for shape and scale endmember changes while enforcing a smooth spectral/spatial variation. The ME formulation takes into account the effect of outliers and copes with some types of EV and NL. The known constraints on the parameter of each observation model are modeled via suitable priors. The posterior distribution associated with each Bayesian model is optimized using a coordinate descent algorithm which allows the computation of the maximum a posteriori estimator of the unknown model parameters. The proposed mixture and Bayesian models and their estimation algorithms are validated on both synthetic and real images showing competitive results regarding the quality of the inferences and the computational complexity when compared to the state-of-the-art algorithms.

==> images/bio_bioucas_short_03_2016.tex <==
Jos\'e Bioucas-Dias (SM'15) received the EE, MSc, PhD, and ``Agregado" degrees from Instituto Superior T\'ecnico (IST), Technical University of Lisbon (TULisbon, now University of Lisbon), Portugal, in 1985, 1991, 1995, and 2007, respectively, all in electrical and computer engineering.

Since 1995, Jos\'e Bioucas-Dias has been with the Department of Electrical and Computer Engineering, IST, where he was an Assistant Professor from 1995 to 2007 and an Associate Professor since 2007. Since 1993, he is also a Senior Researcher with the Pattern and Image Analysis group of the Instituto de Telecomunica\c{c}\~oes, which is a private  non-profit research institution. His  research interests include inverse problems, signal and image processing, pattern recognition, optimization, and remote sensing. His research work has been highly cited and he is included in Thomson Reuters' Highly Cited Researchers 2015 list. 



Jos\'e Bioucas-Dias was an Associate Editor for the {\sc IEEE Transactions on Circuits and Systems} (1997-2000) and  {\sc IEEE Transactions on Image Processing} (2010-2014) and he is  a Senior Area  Editor for the {\sc IEEE Transactions on Image Processing} and an Associate Editor for the {\sc IEEE Transactions on Geoscience and Remote Sensing}.  He was the General Co-Chair of the 3rd IEEE GRSS Workshop on Hyperspectral Image and Signal Processing, Evolution in Remote sensing (WHISPERS'2011) and has been a member of program/technical committees of several international conferences. 



